Explicit Use of Fourier Spectrum in Generative Adversarial Networks

Generative Adversarial Networks have got the researchers' attention due to their state-of-the-art performance in generating new images with only a dataset of the target distribution. It has been shown that there is a dissimilarity between the spectrum of authentic images and fake ones. Since the Fourier transform is a bijective mapping, saying that the model has a significant problem in learning the original distribution is a fair conclusion. In this work, we investigate the possible reasons for the mentioned drawback in the architecture and mathematical theory of the current GANs. Then we propose a new model to reduce the discrepancies between the spectrum of the actual and fake images. To that end, we design a brand new architecture for the frequency domain using the blueprint of geometric deep learning. Then, we experimentally show promising improvements in the quality of the generated images by considering the Fourier domain representation of the original data as a principal feature in the training process.

==> abbreviations.tex <==
% Abbreviations 
% \begin{abbreviations}
% \begin{table}[h!]
%   \caption{Abbreviations list}
%   \label{tab:abb1}
%   \begin{center}
%   \begin{tabular}{cl}
%     \toprule
%     Abbreviation & Full form\\
%     \midrule
%     FFT & Fast Fourier Transform \\
%     DFT & Discrete Fourier Transform\\
%     iFFT & inverse Fast Fourier Transform \\
%     iDFT & inverse Discrete Fourier Transform\\
%     AI & Artificial Intelligence \\
%     ANN & Artificial Neural Networks\\
%     NN &  Neural Networks\\
%     GAN & Generative Adversarial Networks\\
%     CNN & Convolutional Neural Networks \\
%     MLP & Multi Layer Perceptron\\
%     RGB & Red Green Blue (image contex)\\
%   \bottomrule
% \end{tabular}
% \end{center}
% \end{table}

% \begin{table}[ht]
%   \caption{Abbreviations list}
%   \label{tab:abb2}
%   \begin{center}
%   \begin{tabular}{cl}
%     \toprule
%     Abbreviation & Full form\\
%     \midrule
%     FID & Fréchet inception distance\\
%     IS & Inception Score\\
%     KL-divergence & Kullback–Leibler divergence\\
%     EM-distance & Earth Mover's Distance\\
%     CVPR & Conference on Computer Vision and Pattern Recognition\\
%     DCT & Discrete cosine transform\\
%     CPU & Central Processing Unit\\
%     GPU & Graphical Processing Unit\\
%     GDL & Geometric Deep Learning\\
%     i.i.d & Independent and Identically Distributed\\
%     SVM & Support Vector Machines\\
%     FC & Fully Connected\\
%     BN & Batch Norm\\
%     ReLU & Rectified Linear Unit\\
%   \bottomrule
% \end{tabular}
% \end{center}
% \end{table}

\begin{center}
\begin{longtable}{|l l|}
\caption{Abbreviations list} \label{tab:abb_list} \\

\hline \multicolumn{1}{|l}{\textbf{Abbreviation}} & \multicolumn{1}{l|}{\textbf{Full form}} \\ \hline 
\endfirsthead

\multicolumn{2}{l}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline \multicolumn{1}{|l}{\textbf{Abbreviation}} & \multicolumn{1}{l|}{\textbf{Full form}} \\ \hline 
\endhead

\hline \multicolumn{2}{|r|}{{Continued on next page}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

FFT & Fast Fourier Transform \\
DFT & Discrete Fourier Transform\\
iFFT & Inverse Fast Fourier Transform \\
iDFT & Inverse Discrete Fourier Transform\\
AI & Artificial Intelligence \\
ANN & Artificial Neural Networks\\
NN &  Neural Networks\\
GAN & Generative Adversarial Networks\\
CNN & Convolutional Neural Networks \\
MLP & Multi Layer Perceptron\\
RGB & Red Green Blue (image contex)\\
FID & Fréchet Inception Distance\\
IS & Inception Score\\
KL-divergence & Kullback–Leibler divergence\\
EM-distance & Earth Mover's Distance\\
CVPR & Conference on Computer Vision and Pattern Recognition\\
DCT & Discrete Cosine Transform\\
CPU & Central Processing Unit\\
GPU & Graphical Processing Unit\\
GDL & Geometric Deep Learning\\
i.i.d & Independent and Identically Distributed\\
SVM & Support Vector Machines\\
FC & Fully Connected\\
BN & Batch Norm\\
ReLU & Rectified Linear Unit\\

\end{longtable}
\end{center}


==> abstract.tex <==
% Abstract
% \begin{abstract}
Generative Adversarial Networks have got the researchers' attention due to their state-of-the-art performance in generating new images with only a dataset of the target distribution. It has been shown that there is a dissimilarity between the spectrum of authentic images and fake ones. Since the Fourier transform is a bijective mapping, saying that the model has a significant problem in learning the original distribution is a fair conclusion. In this work, we investigate the possible reasons for the mentioned drawback in the architecture and mathematical theory of the current GANs. Then we propose a new model reducing the discrepancies between the spectrum of the actual and fake images. To that end, we design a brand new architecture for the frequency domain using the blueprint of geometric deep learning. Then, we experimentally show that promising improvements in the quality of the generated images by considering the Fourier domain representation of the original data as a principal feature in the training process.

==> acknowledgements.tex <==
% Acknowledgements
% \begin{Acknowledgements}
I would like to express my gratitude to my supervisor, Prof. Hui Jiang, whose guidance was always a light throughout all the project sections. I wish to extend my special thanks to Mr. Behnam (Ben) Asadi, my great friend and colleague at Laboratory for Neural Computing and Machine Learning (NCML), who played a significant role in developing the ideas leading to this thesis. I would like to thank my roommate, Mr. Fazel (Alex) Arasteh from the data mining laboratory of York University, for his assistance in the implementation sections of this project and his constant valuable advice.
